Variance-based sensitivity analysis for time-dependent processes

The global sensitivity analysis of time-dependent processes requires history-aware approaches. We develop for that purpose a variance-based method that leverages the correlation structure of the problems under study and employs surrogate models to accelerate the computations. The errors resulting from fixing unimportant uncertain parameters to their nominal values are analyzed through a priori estimates. We illustrate our approach on a harmonic oscillator example and on a nonlinear dynamic cholera model.

==> pce_gsa.tex <==
\subsection{Definition of the index set $\mathcal{K}_i$}

Here we briefly explain the definition of the index set $\mathcal{K}_i$
in~\eqref{equ:MMM}.
We work with a multivariate PC basis that is 
obtained through a tensor product of appropriate
one-dimensional bases.  More precisely, if we denote by $\{\psi_j(\xi_i)\}_{j =
1}^\infty$ the one-dimensional orthogonal polynomial basis corresponding to
$\xi_i$, we
form the multivariate PC basis $\{\Psi_k\}_{k = 0}^\infty$ as follows: 
\begin{equation}\label{equ:multivariatePC}
	\Psi_k(\xx) = \prod_{i=1}^{\dim} \psi_{\alpha_i^k}(\xi_i), \qquad \xx \in \Omega,
\end{equation}
where $\alpha^k = \left( \alpha_1^k, \alpha_2^k, \cdots, \alpha_d^k\right)$ is
a multi-index, and $\alpha_i^k$ indicates the order of the 1D polynomials in
$\xi_i$.  For example, if $\xi_i$ is standard normal, then $\psi_{\alpha_i^k}$
is the Hermite polynomial of order $\alpha_i^k$.
%
In computer implementations, we will approximate $X(\xx)$ with a truncated series,
\begin{align}\label{eq:FiniteExpansion}
	X(\xx) \approx \sum_{k=0}^{P} c_k \Psi_k(\xx)
\end{align}
where $P$ is specified based on the choice of truncation strategy. In the
present work, we consider truncations based on the total degree of the
polynomials in the series. In this case, letting $p$ be the largest (total)
polynomial degree allowed in the expansion, it is straightforward to show that
$P = (\dim+p)!/(\dim!\,p!)-1$, where as before $\dim$ is the dimension of the
uncertain parameter vector $\xx$.

